CONGRA: Benchmarking Automatic Conflict Resolution

Resolving conflicts from merging different software versions is a challenging task. To reduce the overhead of manual merging, researchers develop various program analysis-based tools which only solve specific types of conflicts and have a limited scope of application. With the development of language models, researchers treat conflict code as text, which theoretically allows for addressing almost all types of conflicts. However, the absence of effective conflict difficulty grading methods hinders a comprehensive evaluation of large language models (LLMs), making it difficult to gain a deeper understanding of their limitations. Furthermore, there is a notable lack of large-scale open benchmarks for evaluating the performance of LLMs in automatic conflict resolution. To address these issues, we introduce ConGra, a CONflict-GRAded benchmarking scheme designed to evaluate the performance of software merging tools under varying complexity conflict scenarios. We propose a novel approach to classify conflicts based on code operations and use it to build a large-scale evaluation dataset based on 44,948 conflicts from 34 real-world projects. We evaluate state-of-the-art LLMs on conflict resolution tasks using this dataset. By employing the dataset, we assess the performance of multiple state-of-the-art LLMs and code LLMs, ultimately uncovering two counterintuitive yet insightful phenomena. ConGra will be released at https://github.com/HKU-System-Security-Lab/ConGra.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See ~\autoref{sc:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See ~\autoref{sc:discussion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerNo{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Abstract.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See ~\autoref{sc:setting}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See ~\autoref{sc:setting}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See ~\autoref{sc:license}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNo{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{}
\end{enumerate}

\end{enumerate}

==> sections/related_work.tex <==
\section{Related Works}

\textbf{Automatic conflict resolution.}
\begin{enumerate}
    \item \textbf{Program analysis approaches.} Spork~\cite{spork} extends the 3DM~\cite{lindholm2004three} merging algorithm to maintain code format and language-specific constructs.
    %
    Mastery~\cite{mastery} introduces a structured merging algorithm using top-down and bottom-up traversal to minimize redundant computations and efficiently handle relocated code.
    %
    SafeMerge~\cite{safemerge} uses a verification algorithm to analyze and combine distinct edits, ensuring conflict-free merged code.
    %
    Intellimerge~\cite{intellimerge} converts source code into a program element graph for semantic analysis, merges matching vertices, and translates the graph back into source code.
    %
    FSTMerge~\cite{fstmerge} is an early framework for semi-structured merging.
    %
    JDime~\cite{jdime} offers a structured merge approach with auto-tuning, dynamically switching between unstructured and structured merging based on conflicts.
    \item \textbf{Machine learning approaches.} MergeBERT~\cite{MergeBERT} treats conflict resolution as a classification problem, using token-level three-way differencing and a transformer encoder model to build a neural program merge framework.
    %
    DeepMerge~\cite{deepmerge} offers the first data-driven approach to resolving merge conflicts with a machine learning model, combining an edit-aware embedding of merge inputs and a variation of pointer networks.
    %
    Gmerge~\cite{gmerge} explores automated merge conflict resolution through k-shot learning with pre-trained large language models (LLMs) like GPT-3~\cite{floridi2020gpt}.
    %
    MergeGen~\cite{mergegen} approaches conflict resolution as a generation task, creating new code that doesn't exist in the input for more flexible combinations.
\end{enumerate}

\textbf{Merge Conflict Benchmark.} 
\begin{enumerate}
    \item \textbf{Merge conflict dataset.} IntelliMerge, FSTMerge, SafeMerge, JDIME, DeepMerge, GMerge and Mastery~\cite{intellimerge, fstmerge, safemerge, jdime, mastery, deepmerge, gmerge} collected evaluation datasets on their own. 
    %
    They crawl merging scenarios from open-source projects in Github.
    %
    Sport~\cite{spork} filtered projects with more than 50 stars and 2 core contributors from existing dataset REAPER~\cite{reaper}.
    %
    MergeGen~\cite{mergegen} follows the datasets generated from MergeBERT~\cite{MergeBERT}.
    \item \textbf{Merge conflict benchmark.} To the best of our knowledge, the only conflict resolving benchmark research is ConflictBench~\cite{shen2024conflictbench}.
    %
    It targets only on Java projects with merely 180 merging scenarios.
    %
    ConflictBench classifies these merging scenarios by the types of developers' resolution, and uses three different metrics with exact string matching algorithm to evaluate software merging tools. 
\end{enumerate}

==> tables/stat_dataset.tex <==
\begin{table}[]
\caption{The number of merge conflict types in the dataset.}
\label{tb:dataset_statistics}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|ccccccc|r@{}}
\toprule
Conflict Type & Text & Text+Syntax & Text+Syntax+Functional & Text+Functional & Syntax & Syntax+Functional & Functional & \multicolumn{1}{l}{Sum} \\ \midrule
Python        & 3051 & 392         & 3062                   & 3027            & 1368   & 431               & 2504       & 13835                   \\
Java          & 1685 & 184         & 725                    & 174             & 2102   & 2104              & 3497       & 10471                   \\
C             & 733  & 825         & 1493                   & 1283            & 3022   & 1231              & 6050       & 14637                   \\
C++           & 357  & 300         & 1371                   & 604             & 774    & 745               & 1854       & 6005                    \\ \bottomrule
\end{tabular}
}
\end{table}
